A Large Population of Luminous Active Galactic Nuclei Lacking X-ray Detections: Evidence for Heavy Obscuration?

We present a large sample of infrared-luminous candidate active galactic nuclei (AGNs) that lack X-ray detections in Chandra, XMM-Newton, and NuSTAR fields. We selected all optically detected SDSS sources with redshift measurements, combined additional broadband photometry from WISE, UKIDSS, 2MASS, and GALEX, and modeled the spectral energy distributions (SEDs) of our sample sources. We parameterize nuclear obscuration in our SEDs with $E(B\!-\!V)_{\text{AGN}}$ and uncover thousands of powerful obscured AGNs that lack X-ray counterparts, many of which are identified as AGN candidates based on straightforward WISE photometric criteria. Using the observed luminosity correlation between restframe 2-10 keV ($L_{\text{X}}$) and restframe AGN 6 $\mu{\text{m}}$ ($L_{\text{MIR}}$), we estimate the intrinsic X-ray luminosities of our sample sources and combine these data with flux limits from X-ray catalogs to determine lower limits on nuclear obscuration. Using the ratio of intrinsic-to-observed X-ray luminosity ($R_{L_{\text{X}}}$), we find a significant fraction of sources with column densities approaching $N_{\text{H}}>$ 10$^{\text{24}}$ cm$^{-{\text{2}}}$, suggesting that multiwavelength observations are necessary to account for the population of heavily obscured AGNs. We simulate the underlying $N_{\text{H}}$ distribution for the X-ray non-detected sources in our sample through survival analysis, and confirm the presence of AGN activity via X-ray stacking. Our results point to a considerable population of extremely obscured AGNs undetected by current X-ray observatories.

==> A Population of X-ray Lacking AGNs/my_commands.tex <==
%% Instruments
\newcommand{\chandra}{\emph{Chandra}\xspace}
\newcommand{\xmmn}{\emph{XMM-Newton}\xspace}
\newcommand{\xmm}{\emph{XMM}\xspace}
\newcommand{\nustar}{\emph{NuSTAR}\xspace}
\newcommand{\galex}{\emph{GALEX}\xspace}
\newcommand{\wise}{\emph{WISE}\xspace}
\newcommand{\xdqso}{XDQSO\emph{z}\xspace}
\newcommand{\chanmaster}{\textsc{chanmaster}\xspace}
\newcommand{\xmmmaster}{\textsc{xmmmaster}\xspace}
\newcommand{\numaster}{\textsc{numaster}\xspace}
\newcommand{\borus}{\textsc{borus}\xspace}
%% Parameters
\newcommand{\chisq}{$\chi^{\text{2}}$\xspace}
\newcommand{\chisqred}{$\chi_{\text{red}}^{\text{2}}$\xspace}
\newcommand{\ebv}{$E(\bv)_{\text{AGN}}$\xspace}
\newcommand{\w}[1]{\emph{W}#1\xspace}
\newcommand{\nh}{$N_{\text{H}}$\xspace}
\newcommand{\lx}{$L_{\text{X}}\xspace$}
\newcommand{\lxlim}{$L_{\text{X,lim}}$\xspace}
\newcommand{\lir}{$L_{\text{MIR}}$\xspace}
\newcommand{\lxir}{$L_{\text{X}}(L_{\text{MIR}})$\xspace}
\newcommand{\rlum}{$R_{L_{\text{X}}}$\xspace}
\newcommand{\llim}{$L_{{\text{X}}_{\text{lim}}}$\xspace}
%% Units
\newcommand{\kev}{\,{\text{keV}}\xspace}
\newcommand{\mum}{\,\mu{\text{m}}\xspace}
\newcommand{\cmcm}{cm$^{-{\text{2}}}$\xspace}
%% Sample Numbers (initial)
\newcommand{\ninit}{3,108,935\xspace}
\newcommand{\nisdss}{3,062,042\xspace}
\newcommand{\nizsupp}{570\xspace}
\newcommand{\nixdqso}{46,893\xspace}
\newcommand{\nioptical}{3,108,935\xspace}
\newcommand{\niwise}{3,108,935\xspace}
\newcommand{\niunwise}{3,108,723\xspace}
\newcommand{\nimir}{3,108,935\xspace}
\newcommand{\niukidss}{952,866\xspace}
\newcommand{\nitwom}{176,692\xspace}
\newcommand{\ninir}{1,068,445\xspace}
\newcommand{\nigalex}{322,527\xspace}
\newcommand{\nixray}{3,108,890\xspace}
\newcommand{\nicha}{365,678\xspace}
\newcommand{\nixmm}{2,888,356\xspace}
\newcommand{\ninst}{45,985\xspace}
\newcommand{\nichaxmm}{158,173\xspace}
\newcommand{\nichanst}{11,802\xspace}
\newcommand{\nixmmnst}{32,497\xspace}
%% Property cuts
\newcommand{\nzgood}{1,600,931\xspace}
\newcommand{\nzgoodtotf}{48.5\%\xspace}
\newcommand{\nrzgood}{1,600,931\xspace}
\newcommand{\nzgoodcumf}{48.5\%\xspace}
\newcommand{\nclean}{2,398,034\xspace}
\newcommand{\ncleantotf}{22.9\%\xspace}
\newcommand{\nrclean}{1,458,103\xspace}
\newcommand{\ncleancumf}{53.1\%\xspace}
\newcommand{\nbands}{1,407,768\xspace}
\newcommand{\nbandstotf}{54.7\%\xspace}
\newcommand{\nrbands}{960,373\xspace}
\newcommand{\nbandscumf}{69.1\%\xspace}
\newcommand{\nfourw}{98,186\xspace}
\newcommand{\nfourwtotf}{96.8\%\xspace}
\newcommand{\nrfourw}{60,994\xspace}
\newcommand{\nfourwcumf}{98.0\%\xspace}
\newcommand{\nnomsk}{2,108,427\xspace}
\newcommand{\nnomsktotf}{32.2\%\xspace}
\newcommand{\nrnomsk}{40,944\xspace}
\newcommand{\nnomskcumf}{98.7\%\xspace}
\newcommand{\nnodup}{3,108,878\xspace}
\newcommand{\nnoduptotf}{\textless0.01\%\xspace}
\newcommand{\nrnodup}{40,935\xspace}
\newcommand{\nnodupcumf}{98.7\%\xspace}
%% Sample Numbers (final)
\newcommand{\nfinal}{40,935\xspace}
\newcommand{\nsdss}{40,349\xspace}
\newcommand{\nzsupp}{168\xspace}
\newcommand{\nxdqso}{586\xspace}
\newcommand{\noptical}{40,935\xspace}
\newcommand{\nwise}{40,935\xspace}
\newcommand{\nunwise}{40,934\xspace}
\newcommand{\nmir}{40,935\xspace}
\newcommand{\nukidss}{11,887\xspace}
\newcommand{\ntwom}{15,236\xspace}
\newcommand{\nnir}{22,373\xspace}
\newcommand{\ngalex}{18,681\xspace}
%% Quality cuts for analysis
\newcommand{\ngal}{7,480\xspace}
\newcommand{\nagn}{33,455\xspace}
\newcommand{\ndet}{4,083\xspace}
\newcommand{\nnon}{36,852\xspace}
\newcommand{\nqgal}{0\xspace}
\newcommand{\nqagn}{3,483\xspace}
\newcommand{\nqdet}{317\xspace}
\newcommand{\nqnon}{3,166\xspace}
%% WISE AGNs
\newcommand{\ninfwac}{4,729\xspace}
\newcommand{\ndetwac}{1,820\xspace}
\newcommand{\nnonwac}{2,909\xspace}
\newcommand{\nqinfwac}{541\xspace}
\newcommand{\nqdetwac}{216\xspace}
\newcommand{\nqnonwac}{325\xspace}
%% Chandra
\newcommand{\ninfcha}{5,939\xspace}
\newcommand{\ndetcha}{595\xspace}
\newcommand{\nnoncha}{5,344\xspace}
\newcommand{\nqinfcha}{1,197\xspace}
\newcommand{\nqdetcha}{97\xspace}
\newcommand{\nqnoncha}{1,100\xspace}
%% XMM
\newcommand{\ninfxmm}{37,146\xspace}
\newcommand{\ndetxmm}{3,424\xspace}
\newcommand{\nnonxmm}{33,722\xspace}
\newcommand{\nqinfxmm}{2,239\xspace}
\newcommand{\nqdetxmm}{216\xspace}
\newcommand{\nqnonxmm}{2,023\xspace}
%% NuSTAR
\newcommand{\ninfnst}{701\xspace}
\newcommand{\ndetnst}{38\xspace}
\newcommand{\nnonnst}{663\xspace}
\newcommand{\nqinfnst}{47\xspace}
\newcommand{\nqdetnst}{4\xspace}
\newcommand{\nqnonnst}{43\xspace}
% Extraneous numbers
\newcommand{\nsrc}{40,935\xspace}
\newcommand{\nqwac}{541\xspace}
\newcommand{\nqres}{2,942\xspace}
\newcommand{\nqdetres}{101\xspace}
\newcommand{\nqnonres}{2,841\xspace}
\newcommand{\nnqual}{3,166\xspace}
\newcommand{\pukidss}{29\%\xspace}
\newcommand{\ptwom}{26\%\xspace}
\newcommand{\pgalex}{43\%\xspace}
\newcommand{\pcorr}{${\sim}$7\%\xspace}
\newcommand{\lcorr}{$-$0.039$\pm$0.064\xspace}
\newcommand{\pctwagn}{${\sim}$17\%\xspace}
\newcommand{\nages}{16,014\xspace}
\newcommand{\nexages}{14,965\xspace}
\newcommand{\ninages}{1,049\xspace}
\newcommand{\nexoff}{29\xspace}
\newcommand{\zexsig}{0.057\xspace}
\newcommand{\zinsig}{0.046\xspace}


==> A Population of X-ray Lacking AGNs/table1.tex <==
\begin{deluxetable*}{lrrrrrrrrrr}
\tablecaption{Number of sources with various telescope coverage.\label{sample}}
\tablehead{\colhead{} & \colhead{SDSS} & \colhead{\xdqso} & \colhead{\wise} & \colhead{UKIDSS} & \colhead{2MASS} & \colhead{\galex} & \colhead{\chandra} & \colhead{\xmm} & \colhead{\nustar}}
\startdata
Initial & \nisdss & \nixdqso & \niwise & \niunwise & \nitwom & \nigalex & \nicha   & \nixmm   & \ninst   \\
Final   & \nsdss  & \nxdqso  & \nwise  & \nunwise  & \ntwom  & \ngalex  & \ninfcha & \ninfxmm & \ninfnst \\
\enddata
\tablecomments{Our initial sample of \ninit sources with optical and IR coverage, reduced to \nfinal sources for our final sample. All \wise photometry was replaced with forced photometry from unWISE where available (\niunwise initial, \nunwise final).}
\end{deluxetable*}


==> A Population of X-ray Lacking AGNs/table2.tex <==
\begin{deluxetable*}{lrrrr}
\tablecaption{Various property selection criteria and effects on sample numbers.\label{prop_cuts}}
\tablehead{\colhead{Property Cut} & \colhead{$N_{\text{tot}}$} & \colhead{Tot. Loss} & \colhead{$N_{\text{cum}}$} & \colhead{Cum. Loss}}
\startdata
initial sample          & \ninit  & 0\%         & \ninit   & 0\%         \\
valid redshift          & \nzgood & \nzgoodtotf & \nrzgood & \nzgoodcumf \\
clean photometry        & \nclean & \ncleantotf & \nrclean & \ncleancumf \\
seven photometric bands & \nbands & \nbandstotf & \nrbands & \nbandscumf \\
four \wise bands        & \nfourw & \nfourwtotf & \nrfourw & \nfourwcumf \\
not removed by mask     & \nnomsk & \nnomsktotf & \nrnomsk & \nnomskcumf \\
not a duplicate         & \nnodup & \nnoduptotf & \nrnodup & \nnodupcumf \\
\enddata
\tablecomments{Individual and cumulative effect of each property cut on our sample. For each property cut, the first two subsequent columns list the number of sources which pass the designated cut and the fractional loss from our initial sample (\ninit sources). The last two columns track the cumulative effects of each property cut on sample size and our cumulative fractional loss.}
\end{deluxetable*}


==> A Population of X-ray Lacking AGNs/table3.tex <==
\begin{deluxetable*}{rrrrrrrrr}
\tablecolumns{9}
\tablecaption{Source positions and X-ray luminosity estimates by observatory.\label{xlum}}
\tablehead{\colhead{SDSS ObjID} & \colhead{RA} & \colhead{Dec} & \colhead{$\log L_{\text{X}}(\chandra)$} & \colhead{$\log L_{\text{X}}(\xmm)$} & \colhead{$\log L_{\text{X}}(\nustar)$} & \colhead{} \\
\colhead{} & \colhead{[deg]} & \colhead{[deg]} & \colhead{[erg\,s$^{-1}$]} & \colhead{[erg\,s$^{-1}$]} & \colhead{[erg\,s$^{-1}$]} & \colhead{}}
\startdata
1237667223933550815 &   4.7399 & -20.3684 &           \nodata &    43.11$\pm$0.09 &           \nodata &     XMM \\
1237667223399170264 &  10.7800 & -20.6891 & $<$41.25$\pm$0.16 & $<$41.81$\pm$0.16 &           \nodata &     CHA \\
1237667223399170855 &  10.8610 & -20.5961 & $<$42.46$\pm$0.15 & $<$43.03$\pm$0.15 &           \nodata &     CHA \\
1237667223399170348 &  10.7717 & -20.6602 &           \nodata &    44.28$\pm$0.09 &           \nodata &     XMM \\
1237667223387439337 & 342.3175 & -19.3099 &           \nodata & $<$41.47$\pm$0.15 &           \nodata &     XMM \\
1237667223387504664 & 342.4005 & -19.2649 &           \nodata & $<$40.37$\pm$0.21 &           \nodata &     XMM \\
1237671166167941234 & 166.6228 & -18.3672 &           \nodata &    44.01$\pm$0.06 &           \nodata &     XMM \\
1237667225535119631 & 343.0232 & -17.7923 &           \nodata & $<$41.42$\pm$0.17 &           \nodata &     XMM \\
1237667223389471530 & 347.1830 & -19.8406 &           \nodata & $<$43.05$\pm$0.15 &           \nodata &     XMM \\
1237667225544556806 &   5.6148 & -18.9625 &           \nodata & $<$42.67$\pm$0.15 & $<$43.06$\pm$0.15 &     XMM \\
\enddata
\tablecomments{Upper limit X-ray luminosity estimates are labeled by ``$<$'. The field chosen for our analysis is shown in the final column.}
%\tablerefs{}
\end{deluxetable*}


==> A Population of X-ray Lacking AGNs/table4.tex <==
\begin{deluxetable*}{rrrrrrrrr}
\tablecolumns{9}
\tablecaption{SED modeling output parameters.\label{sed_output}}
\tablehead{\colhead{$z$} & \colhead{$E(\bv)_{\text{AGN}}$} & \colhead{$C_{\text{AGN}}$} & \colhead{$C_{\text{ELL}}$} & \colhead{$C_{\text{SFG}}$} & \colhead{$C_{\text{IRR}}$} & \colhead{$\chi^2 /$ DoF} & \colhead{$P_{\text{AGN}}$} & \colhead{$\log L_{\text{MIR}}$} \\
\colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{} & \colhead{[\%]} & \colhead{[erg\,s$^{-1}$]}}
\startdata
0.348$\pm$0.039 &  6.21$\pm$2.91 & 5.04$\times$10$^{-17}$ & 7.22$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 1.17$\times$10$^{-16}$ &  14.61 / 4 & 100 & 44.05$\pm$0.07 \\ 
0.112$\pm$0.030 & 50.00$\pm$0.50 & 5.32$\times$10$^{-17}$ & 1.22$\times$10$^{-15}$ & 0.00$\times$10$^{+00}$ & 1.53$\times$10$^{-16}$ &  27.09 / 8 &  86 & 43.06$\pm$0.01 \\ 
0.391$\pm$0.060 &  6.98$\pm$2.61 & 6.14$\times$10$^{-17}$ & 0.00$\times$10$^{+00}$ & 9.47$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ &  38.95 / 5 & 100 & 44.24$\pm$0.10 \\ 
0.778$\pm$0.172 &  0.06$\pm$0.00 & 7.05$\times$10$^{-17}$ & 3.93$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 0.00$\times$10$^{+00}$ &  30.68 / 6 & 100 & 44.92$\pm$0.13 \\ 
0.180$\pm$0.030 & 35.38$\pm$4.33 & 7.49$\times$10$^{-17}$ & 9.09$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 1.38$\times$10$^{-16}$ &  19.44 / 6 &  97 & 43.63$\pm$0.01 \\ 
0.055$\pm$0.017 & 25.02$\pm$3.06 & 1.86$\times$10$^{-16}$ & 3.19$\times$10$^{-15}$ & 7.72$\times$10$^{-16}$ & 5.65$\times$10$^{-16}$ &  53.70 / 6 & 100 & 42.98$\pm$0.05 \\ 
0.555$\pm$0.088 &  0.04$\pm$0.00 & 9.47$\times$10$^{-17}$ & 2.65$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 5.04$\times$10$^{-17}$ &  57.13 / 6 & 100 & 44.75$\pm$0.10 \\ 
0.096$\pm$0.034 & 50.00$\pm$0.50 & 9.97$\times$10$^{-17}$ & 6.61$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 1.69$\times$10$^{-16}$ &   9.59 / 5 & 100 & 43.20$\pm$0.01 \\ 
0.367$\pm$0.051 & 50.00$\pm$0.50 & 1.25$\times$10$^{-16}$ & 3.68$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 2.31$\times$10$^{-17}$ &  26.89 / 3 &  97 & 44.50$\pm$0.01 \\ 
0.328$\pm$0.115 & 39.71$\pm$5.45 & 7.65$\times$10$^{-17}$ & 1.79$\times$10$^{-16}$ & 0.00$\times$10$^{+00}$ & 2.71$\times$10$^{-17}$ &   1.56 / 3 &  98 & 44.18$\pm$0.02 \\ 
\enddata
\tablecomments{Modeling output parameters redshift, color excess \ebv, template normalizations (AGN, elliptical, star-forming, irregular/starburst), chi-squared per degrees of freedom, percentage of resampled realizations with AGN contribution ($C_{\text{AGN}} > 0$), and AGN $6\mum$ luminosity. Uncertainties on \ebv and $\log L_{\text{IR}}$ were estimated via the median absolute deviation of all source realizations containing AGN contribution.}
%\tablerefs{}
\end{deluxetable*}


==> A Population of X-ray Lacking AGNs/table5.tex <==
\begin{deluxetable}{llrr}
\tablecolumns{3}
\tablecaption{Number of sources with various selections.\label{qual_cut}}
\tablehead{\colhead{Selection} & & \colhead{$N_{\text{final}}$} & \colhead{$N_{\text{subset}}$}}
\startdata
\multirow{4}{*}{Final sample} & SED Galaxy     & \ngal    & \nqgal    \\
                              & SED Galaxy+AGN & \nagn    & \nqagn    \\
                              & X-ray detected & \ndet    & \nqdet    \\
                              & X-ray non-det. & \nnon    & \nqnon    \\
                              \cline{2-4}
\multirow{3}{*}{\wise AGN}    & in catalog     & \ninfwac & \nqinfwac \\
                              & X-ray detected & \ndetwac & \nqdetwac \\
                              & X-ray non-det. & \nnonwac & \nqnonwac \\
                              \cline{2-4}
\multirow{3}{*}{\chandra}     & in X-ray field & \ninfcha & \nqinfcha \\
                              & X-ray detected & \ndetcha & \nqdetcha \\
                              & X-ray non-det. & \nnoncha & \nqnoncha \\
                              \cline{2-4}
\multirow{3}{*}{\xmm}         & in X-ray field & \ninfxmm & \nqinfxmm \\
                              & X-ray detected & \ndetxmm & \nqdetxmm \\
                              & X-ray non-det. & \nnonxmm & \nqnonxmm \\
                              \cline{2-4}
\multirow{3}{*}{\nustar}      & in X-ray field & \ninfnst & \nqinfnst \\
                              & X-ray detected & \ndetnst & \nqdetnst \\
                              & X-ray non-det. & \nnonnst & \nqnonnst \\
\enddata
\tablecomments{Our final sample of \nsrc sources, reduced to \nqagn sources for our analysis subset.}
%\tablerefs{}
\end{deluxetable}


==> A Population of X-ray Lacking AGNs/table6.tex <==
\begin{deluxetable*}{lrrrrrrr}
\tablecolumns{8}
\tablecaption{X-ray stacking data and results.\label{stack_results}}
\tablehead{
\colhead{} & \colhead{$t_{\text{exp}}$} & \colhead{Energy} & \colhead{$N_{\text{src}}$} & \colhead{$N_{\text{bg}}$} & \colhead{$N_{\text{net}}$} & \colhead{$F_{\text{X}}$} & \colhead{$\log L_{\text{X}}$} \\
\colhead{} & \colhead{[Ms]} & \colhead{[keV]} & \colhead{} & \colhead{} & \colhead{} & \colhead{[erg\,s$^{-1}$\,cm$^{-2}$]} & \colhead{[erg\,s$^{-1}$]}
}
\startdata
\multirow{2}{*}{\wise AGN (X-ray det.)}     & \multirow{2}{*}{ 1.34} & 0.5--2 & 7881 &   91 & 7789 & (3.61$\pm$1.00)$\times10^{-14}$ & 43.41$\pm$0.12 \\
                                            &                        & 2--7   & 3856 &  118 & 3737 & (8.45$\pm$1.99)$\times10^{-14}$ & 43.78$\pm$0.10 \\
                                                                     \cline{2-8}
\multirow{2}{*}{\wise AGN (X-ray non-det.)} & \multirow{2}{*}{ 1.48} & 0.5--2 &  118 &   22 &   95 & (3.99$\pm$1.18)$\times10^{-16}$ & 41.54$\pm$0.13 \\
                                            &                        & 2--7   &  117 &   52 &   64 & (1.32$\pm$0.36)$\times10^{-15}$ & 42.05$\pm$0.12 \\
                                                                     \cline{2-8}
\multirow{2}{*}{Secondary (X-ray det.)}     & \multirow{2}{*}{ 1.18} & 0.5--2 & 1516 &   71 & 1444 & (7.60$\pm$2.20)$\times10^{-15}$ & 42.84$\pm$0.13 \\
                                            &                        &   2--7 & 1256 &  110 & 1145 & (2.94$\pm$0.64)$\times10^{-14}$ & 43.42$\pm$0.09 \\
                                                                     \cline{2-8}
\multirow{2}{*}{Secondary (X-ray non-det.)} & \multirow{2}{*}{22.57} & 0.5--2 & 1190 &  801 &  388 & (1.07$\pm$0.14)$\times10^{-16}$ & 40.78$\pm$0.05 \\
                                            &                        &   2--7 & 1210 &  972 &  237 & (3.20$\pm$0.61)$\times10^{-16}$ & 41.25$\pm$0.08 \\
                                                                     \cline{2-8}
\multirow{2}{*}{Removed AGN}                & \multirow{2}{*}{18.51} & 0.5--2 & 1108 &  672 &  435 & (1.46$\pm$0.14)$\times10^{-16}$ & 40.84$\pm$0.04 \\
                                            &                        & 2--7   & 1076 &  847 &  228 & (3.76$\pm$0.80)$\times10^{-16}$ & 41.25$\pm$0.09 \\
                                                                     \cline{2-8}
\multirow{2}{*}{SED galaxy}                 & \multirow{2}{*}{21.67} & 0.5--2 & 1301 &  858 &  442 & (1.27$\pm$0.13)$\times10^{-16}$ & 40.78$\pm$0.05 \\
                                            &                        &   2--7 & 1023 &  970 &   52 & (7.39$\pm$5.63)$\times10^{-17}$ & 40.54$\pm$0.33 \\
\enddata
\tablecomments{X-ray stacking results for energy ranges of \mbox{0.5--2} and \mbox{2--7 keV}. For each energy range, we present exposure time, photon counts, and flux and luminosity estimates. The flux and luminosity values listed in the \mbox{2--7 keV} energy range have been scaled to \mbox{2--10 keV} for direct comparison to the body of this work.}
%\tablerefs{}
\end{deluxetable*}

